Towards Understanding Text Hallucination of Diffusion Models via Local Generation Bias

Score-based diffusion models have achieved incredible performance in generating realistic images, audio, and video data. While these models produce high-quality samples with impressive details, they often introduce unrealistic artifacts, such as distorted fingers or hallucinated texts with no meaning. This paper focuses on textual hallucinations, where diffusion models correctly generate individual symbols but assemble them in a nonsensical manner. Through experimental probing, we consistently observe that such phenomenon is attributed it to the network's local generation bias. Denoising networks tend to produce outputs that rely heavily on highly correlated local regions, particularly when different dimensions of the data distribution are nearly pairwise independent. This behavior leads to a generation process that decomposes the global distribution into separate, independent distributions for each symbol, ultimately failing to capture the global structure, including underlying grammar. Intriguingly, this bias persists across various denoising network architectures including MLP and transformers which have the structure to model global dependency. These findings also provide insights into understanding other types of hallucinations, extending beyond text, as a result of implicit biases in the denoising models. Additionally, we theoretically analyze the training dynamics for a specific case involving a two-layer MLP learning parity points on a hypercube, offering an explanation of its underlying mechanism.

==> redundant.tex <==
\textbf{Lemma} Denote $\Gamma=\{\sigma: [d]\mapsto \{\pm 1\}^d \}$ and $\Gamma^+ = \left\{ \sigma\in \Gamma: \sigma(1)=1, \prod_{i=2}^d \sigma(i)=1 \right\}$. With a little abuse of notation, if a set $\Omega\subseteq \mathbb{R}^d$ satisfies $\sigma(\Omega)=\{\sigma(x): x \in \Omega, \sigma\in \Gamma^+\}=\Omega$. Then we have
\begin{align}
    \mathbb{E}_{x\sim \mc{D}} [ xy^*(x)\mathbb{I}[x\in \Omega] ] \propto e_1.
\end{align}
\textit{Proof.}
\begin{align}
    \mathbb{E}_{x\sim \mc{D}} [ xy^*(x)\mathbb{I}[x\in \Omega] ] &= \int_{x\in \Omega} P_{\mc{D}}(x) \sum_{x_0\in \mc{X}} x\cdot \exp(x^{\top} x_0) \mathrm{d}x \\
    &=\int_{x\in \Omega} P_{\mc{D}}(x) \frac{1}{|\Gamma^+|} \sum_{\sigma\in\Gamma^+} \sum_{x_0\in \mc{X}} \sigma(x) \cdot \exp(\sigma(x)^{\top} \sigma(x_0)) \mathrm{d}x \\
    &=\int_{x\in \Omega} P_{\mc{D}}(x) \mathrm{d}x \frac{1}{|\Gamma^+|} \sum_{\sigma\in\Gamma^+}  \sum_{x_0\in \mc{X}} \sigma(x) \cdot \exp(x^{\top} x_0) \\
    &=\int_{x\in \Omega} P_{\mc{D}}(x)  \mathrm{d}x \frac{1}{|\Gamma^+|} \sum_{x_0\in \mc{X}} \sum_{\sigma\in\Gamma^+}   \sigma(x) \cdot \exp(x^{\top} x_0) \\
    &=\int_{x\in \Omega} P_{\mc{D}}(x) \mathrm{d}x \frac{1}{|\Gamma^+|} \sum_{x_0\in \mc{X}}  \exp(x^{\top} x_0) \underbrace{\sum_{\sigma\in\Gamma^+} \sigma(x)}_{=\lambda e_1} 
\end{align}

\textbf{Theorem 1.} (First Stage Dynamics) \textit{At first stage, we have}
\begin{align}
    f_{\theta(t)}(\bs{x}) = o(1), \quad \langle w_r, e_1 \rangle = 1- o(\text{something}).
\end{align}
If $b_r=0$, we have $G(w_r,b_r)$ is nearly linear in $w_r$ deduced as following. 
\begin{align}
    G(w_r,b_r) =& \mathbb{E}_{x\sim\mc{D}}[y^*(x)\phi(w_r^{\top}x+b_r)] \\
    \approx & \frac{1}{2}\left( \mathbb{E}_{x\sim\mc{D}}[y^*(x)\phi(w_r^{\top}x+0)] + \mathbb{E}_{x \sim \mc{D}}[y^*(x)\phi(w_r^{\top}(-x)+0)] \right) \\
    =& \frac{1}{2} \mathbb{E}_{x\sim\mc{D}} [y^*(x)(\phi(w_r^{\top}x)+\phi(-w_r^{\top}x))] \\
    =& \frac{1+k_{leaky}}{2} \left\langle w_r, \tilde{\mu} \right\rangle,
\end{align}
where $\tilde{\mu}=\mathbb{E}_{x\sim \mc{D}} [x\cdot y^*(x)]$.In consequence 
\begin{align}
     \frac{\mathrm{d} w_r}{\mathrm{d} t} & \propto \mathbb{E}_{x\sim \mc{D}} \left[ xy^*(x) \right] 
\end{align}
% \begin{align}
%     \nabla_{w} \mc{L}=&\mathbb{E}_{x\sim \mc{D}} [ xy^*(x)\phi'(w^{\top}x + b)] \\
%     =& \frac{1}{2}\mathbb{E}_{x\sim \mc{D}} [ xy^*(x)\phi'(w^{\top}x + b) + (-x)y^*(-x)\phi'(w^{\top}(-x) + b)] \\
%     =& \frac{1}{2}\mathbb{E}_{x\sim \mc{D}} [ xy^*(x)(\phi'(w^{\top}x + b) +\phi'(-w^{\top}x + b))] \\
%     =& \mathbb{E}_{x\sim \mc{D}} [ xy^*(x)] + \operatorname{sgn}(b)\mathbb{E}_{x\sim \mc{D}} [xy^*(x)\mathbb{I}[ |w^{\top} x| \leq |b|]]
% \end{align}
% Note that first term is parallel to $e_1$ and it is constant. Thus the deviation of $\nabla_{w} \mc{L}$ from $e_1$ requires bounding the second term.
% \begin{align}
%     &\mathbb{E}_{x\sim \mc{D}} [xy^*(x)\mathbb{I}[ |w^{\top} x| \leq |b|]] \\
%   =&\mathbb{E}_{x\sim \mc{D}} [xy^*(x)\mathbb{I}[ |w_1 x_1 + \langle w_{\perp}, x_{\perp}\rangle | \leq |b|]] \\
%   =&\mathbb{E}_{x\sim \mc{D}} [xy^*(x)\mathbb{I}[ -w_1 x_1-|b|\leq \langle w_{\perp}, x_{\perp} \rangle\leq -w_1 x_1+|b|]] 
% \end{align}
% Observation: For most $x\sim \mc{D}$, $\langle w_{\perp}, x_{\perp} \rangle$ can only vary in range $O(\|w_{\perp}\|)$, which is much smaller than the band width $2|b|$. Therefore, in most $x_1$ slices, either all or none $x_{\perp}$ satisfies $-w_1 x_1-|b|\leq \langle w_{\perp}, x_{\perp} \rangle\leq -w_1 x_1+|b|$. Only when $|w_1x_1|\approx |b|$ can yield marginal expectation significantly deviate from $e_1$.

And if we focus specifically on the $1_{st}$ dimension, it becomes
\begin{align}
    y^*(x)=s_{\alpha,\mc{X}}(x)^{(1)}&= \frac{1}{Z} \sum_{x_i\in\mc{X}} \frac{\sqrt{\alpha}x_{i}^{(1)}-x^{(1)}}{\sqrt{1-\alpha}}\cdot \exp\left( -\frac{\|\sqrt{\alpha}x_i-x\|^2}{2(1-\alpha)} \right).
\end{align}
An important property of this target function is that it is centrosymmetric $y^*(x)+y^*(-x)=0$. It mostly depends on $x[k]$ but also contains a more complex and collective dependency on the remaining entries. 

Finally we bound the difference between the surrogate trajectory $\tilde{\theta}(s)$ and the actual trajectory $\theta(s)$.

\begin{lemma}
    $|K(w,b)|\leq \alphasC$.
\end{lemma}
\begin{proof}
    By symmetry, WLOG we consider the case where $w^{(i)}>0$. Then 
    \begin{align*}
        K(w,b)
        & \leq \frac{\alphasC}{2}\sup_{D\in \R} \frac{1}{\sqrt{1+D^2}}\left(1 +\frac{1}{2} \erf\left(\frac{D}{\sqrt{2(1-\bar{\alpha}_t)}}+\sqrt{\frac{\bar{\alpha}_t}{2(1-\bar{\alpha}_t)}}\right)\right.\\
        & \left.+\frac{1}{2}\erf\left(\frac{D}{\sqrt{2(1-\bar{\alpha}_t)}}-\sqrt{\frac{\bar{\alpha}_t}{2(1-\bar{\alpha}_t)}}\right)\right)\\
        &\leq  \frac{\alphasC}{2} (1+\frac{1}{2} + \frac{1}{2})\\
        & = \alphasC.
\end{align*}
\end{proof}
\begin{lemma}
    With high probability $1-\delta$, $|a_j(0)|\leq \sigma_{init}\sqrt{4(d+r^2)\log (md\delta^{-1})}$ for all $j\in [m]$.
\end{lemma}
\begin{proof}
    Since $w_{j}(0)\sim \mc{N}(0, \sigma_{init}^2)$ and $b_{j}(0)\sim \mc{N}(0, \sigma_{init}^2r^2)$, with probability $\geq 1-\frac{\delta}{dm}$, for a single $j$ there is $\norm{w_j(0)}\leq \sigma_{init}\sqrt{4d\log (md\delta^{-1})}$ and $|b_j(0)|\leq r \sigma_{init}\sqrt{4\log (md\delta^{-1})}$. Then by union bound, using $|a_j(0)|=\sqrt{\norm{w_j(0)}^2 + b_j(0)^2}$, we can prove the result.
\end{proof}

\begin{lemma}
    
\end{lemma}
\begin{proof}
    We know that 
    \begin{align*}
         \frac{d}{ds}a_j &= -2\E_x (s_\theta(x)-y_i(x))\sigma(w_{j}^\top x + b_{j})\\
         & = -2\E_x s_\theta(x)\sigma(w_{j}^\top x + b_{j}) + 2|a_j|K(\frac{w_{j}}{|a_j|},\frac{b_j}{|a_j|}).
    \end{align*}
    Now 
    \begin{align*}
        |\E_x s_\theta(x)\sigma(w_{j}^\top x + b_{j})| & = |\E_x \sum a_k \sigma(w_{k}^\top x + b_{k})\sigma(w_{j}^\top x + b_{j})| \\
        & \leq  \sum_k |a_k| \sqrt{(\E_x  \sigma(w_{k}^\top x + b_{k})^2)(\E_x \sigma(w_{j}^\top x + b_{j})^2)}\\
        & \leq m\sup_k |a_k|  \sqrt{(\E_x  (w_{k}^\top x + b_{k})^2)(\E_x (w_{j}^\top x + b_{j})^2)}\\
        & = m\sup_k |a_k|\sqrt{(\norm{w_k}^2 + b_k^2)(\norm{w_j}^2 + b_j^2)}
    \end{align*}
\end{proof}

